Near-Field Wireless Power Transfer with Dynamic Metasurface Antennas

Radio frequency wireless power transfer (WPT) enables charging low-power mobile devices without relying on wired infrastructure. Current existing WPT systems are typically designed assuming far-field propagation, where the radiated energy is steered in given angles, resulting in limited efficiency and possible radiation in undesired locations. When large arrays at high frequencies, such as DMA, are employed, WPT might take place in the radiating near-field (Fresnel) region where spherical wave propagation holds, rather than plane wave propagation as in the far-field. In this paper, we study WPT systems charging multiple devices in the Fresnel region, where the energy transmitter is equipped with an emerging DMA, exploring how the antenna configuration can exploit the spherical wavefront to generate focused energy beams. In particular, after presenting a mathematical model for DMA-based radiating near-field WPT systems, we characterize the weighted sum-harvested energy maximization problem of the considered system, and we propose an efficient solution to jointly design the DMA weights and digital precoding vector. Simulation results show that our design generates focused energy beams that are capable of improving energy transfer efficiency in the radiating near-field with minimal energy pollution.

==> Near-field WPT_DMA/definitions.tex <==

\newcommand{\df}{d_\mathrm{F}}

\newcommand{\xf}{x_\mathrm{F}}
\newcommand{\yf}{y_\mathrm{F}}
\newcommand{\zf}{z_\mathrm{F}}


\newcommand{\g}{\mathrm{g}}
\newcommand{\Ge}{G_\mathrm{e}}

\newcommand{\p}{\mathbf{p}}
\newcommand{\hpf}{\hat{\mathbf{p}}_\mathrm{F}}
\newcommand{\pf}{\mathbf{p}_\mathrm{F}}
\newcommand{\pil}{\mathbf{p}_{i,l}}
\newcommand{\yil}{{y}_{i,l}}
\newcommand{\Yil}{{Y}_{i,l}}
\newcommand{\Ail}{{A}_{i,l}}
